PolyChopper: a Polyhedron Splitting Scheme

We introduce and implement a novel scheme, called \textit{PolyChopper}, for splitting a convex polyhedron into a finite set of disjoint convex sub-polyhedra. The algorithm cuts the polyhedron with a plane, which can either be prescribed as an external constraint or automatically determined from the inertia tensor. The resulting intersection vertices are then adjusted to control the complexity and quality of the generated elements, introducing additional ``notch wedges'', tetrahedra and pyramids, according to a user-defined quality parameter. Experimental results demonstrate that the proposed approach is robust and consistently produces sub-polyhedra that are both simpler and of higher quality than the original polyhedron. Furthermore, recursively applying the algorithm generates a hierarchy of polyhedral subdivisions with progressively smaller elements, all guaranteed to remain convex and predominantly tetrahedral.

==> A2-thingi.tex <==
We consider the problem of meshing a convex domain by iteratively splitting it in convex parts.
This Section contains preliminary work, and up to our knowledge this algorithm is the first attempt to solve this type of problem in dimension three.

Polyhedra are obtained by the decomposition into convex elements of CAD models through the \texttt{CGAL::convex\_decomposition\_3()} routine~\cite{cgal:eb-26a}, see Figure~\ref{fig:results:polys}(bottom). 
Models are taken from the Thingi10K dataset \cite{Thingi10K}.
Compared to the previous dataset, this represents a particular applicative scenario, in which faces can be both polygonal and with low quality.

\begin{figure}[ht!]
    \centering
    \begin{tabular}{ccc}
        \includegraphics[height=.12\linewidth]{pics/poly_thingi_0.pdf} & 
        \hspace{2em} &
        \includegraphics[height=.12\linewidth]{pics/poly_thingi_1.pdf} 
    \end{tabular}\\
    CAD Polyhedra
    \caption{CAD model decomposed into convex polyhedra.}
    \label{fig:mesh:cad}
\end{figure}
